Turning block-sequential automata networks into smaller parallel networks with isomorphic limit dynamics

We state an algorithm that, given an automata network and a block-sequential update schedule, produces an automata network of the same size or smaller with the same limit dynamics under the parallel update schedule. Then, we focus on the family of automata cycles which share a unique path of automata, called tangential cycles, and show that a restriction of our algorithm allows to reduce any instance of these networks under a block-sequential update schedule into a smaller parallel network of the family and to characterize the number of reductions operated while conserving their limit dynamics. We also show that any tangential cycles reduced by our main algorithm are transformed into a network whose size is that of the largest cycle of the initial network. We end by showing that the restricted algorithm allows the direct characterization of block-sequential double cycles as parallel ones.

==> figures/cycleSequence1.tex <==

\tikzset{smallstate/.style = {state, inner sep=0pt, minimum size=.8cm}}

\centering
\begin{minipage}{.4\textwidth}
\centering
\vspace{.4cm}
\begin{tikzpicture}  [node distance = .5cm, -{Latex[length=1.5mm, width=1.5mm]}]
	\node[smallstate] (A) {a};
	\node[smallstate] (B) [right =of A] {b};
	\node[smallstate] (C) [right =of B] {c};

	\path
			(A) edge [bend right] node [below] {\tiny $\geqslant$} (B)
			(B) edge [bend right] node [above] {\tiny $\geqslant$} (A)
			(C) edge node [above] {\tiny $<$} (B);
			
	
	 \draw (C) to [out=20, in=-20, looseness=7] node [right] {\tiny $\geqslant$} (C);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.3\textwidth}
\centering
  \begin{align*}
    f_a(x) &= x_b \\
    f_b(x) &= x_a \vee x_c \\
    f_c(x) &= x_c
  \end{align*}
\end{minipage}
\begin{minipage}{.2\textwidth}
\centering
 Initial network, $\Delta = (c, ab)$
\end{minipage}

\vspace{.2cm}
\hrulefill
\vspace{-.3cm}


\begin{minipage}{.4\textwidth}
\centering
\vspace{.4cm}
\begin{tikzpicture}  [node distance = .5cm, -{Latex[length=1.5mm, width=1.5mm]}]
	\node[smallstate] (A) {a};
	\node[smallstate] (B) [right =of A] {b};
	\node[smallstate] (C) [right =of B] {c};

	\path
			(A) edge [bend right] (B)
			(B) edge [bend right] (A)
			(C) edge (B);
			
	
	 \draw (C) to [out=20, in=-20, looseness=7] (C);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.3\textwidth}
\centering
  \begin{align*}
    f_a(x) &= x_b \\
    f_b(x) &= x_a \vee x_c \\
    f_c(x) &= x_c
  \end{align*}
\end{minipage}
\begin{minipage}{.2\textwidth}
\centering
 Output of Algorithm~\ref{algo-IAC}
\end{minipage}


==> figures/cycleSequence2.tex <==

\tikzset{smallstate/.style = {state, inner sep=0pt, minimum size=.8cm}}

\centering
\begin{minipage}{.4\textwidth}
\centering
\vspace{.4cm}
\begin{tikzpicture}  [node distance = .5cm, -{Latex[length=1.5mm, width=1.5mm]}]
	\node[smallstate] (A) {a};
	\node[smallstate] (B) [right =of A] {b};
	\node[smallstate] (C) [right =of B] {c};

	\path
			(A) edge [bend right] node [below] {\tiny $\geqslant$} (B)
			(B) edge [bend right] node [above] {\tiny $\geqslant$} (A)
			(C) edge node [above] {\tiny $<$} (B);
			
	
	 \draw (C) to [out=20, in=-20, looseness=7] node [right] {\tiny $\geqslant$} (C);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.3\textwidth}
\centering
  \begin{align*}
    f_a(x) &= x_b \\
    f_b(x) &= x_a \vee x_c \\
    f_c(x) &= x_c
  \end{align*}
\end{minipage}
\begin{minipage}{.2\textwidth}
\centering
 Initial network, $\Delta = (c, ab)$
\end{minipage}

\vspace{.2cm}
\hrulefill
\vspace{-.3cm}


\begin{minipage}{.4\textwidth}
\centering
\vspace{.4cm}
\begin{tikzpicture}  [node distance = .5cm, -{Latex[length=1.5mm, width=1.5mm]}]
	\node[smallstate] (A) {a};
	\node[smallstate] (B) [right =of A] {b};
	\node[smallstate] (C) [right =of B] {c};

	\path
			(A) edge [bend right] (B)
			(B) edge [bend right] (A)
			(C) edge (B);
			
	
	 \draw (C) to [out=20, in=-20, looseness=7] (C);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.3\textwidth}
\centering
  \begin{align*}
    f_a(x) &= x_b \\
    f_b(x) &= x_a \vee x_c \\
    f_c(x) &= x_c
  \end{align*}
\end{minipage}
\begin{minipage}{.2\textwidth}
\centering
 Output of Algorithm~\ref{algo-IAC}
\end{minipage}


==> figures/interactionDigraph.tex <==

\begin{tikzpicture}  [-{Latex[length=1.5mm, width=1.5mm]}, node distance=0.5cm]
	\node[state] (A) {a};
	\node[state] (C) [below right =of A] {c};
	\node[state] (B) [below left =of A] {b};

	\path
			(A) edge (B)
			(A) edge [bend left] (C)
			(C) edge [bend left] (A)
			(B) edge (C);

\end{tikzpicture}


==> figures/moduleInteractionDigraph.tex <==

\begin{tikzpicture}  [-{Latex[length=1.5mm, width=1.5mm]}]
	\node[state] (A) {a};
	\node[state] (C) [below right =of A] {c};
	\node[state] (B) [below left =of A] {b};

	\path
			(A) edge (B)
			(A) edge (C)
			(B) edge (C);

	\node [left =20pt of A] (alpha1) {$\alpha$};
	\draw (alpha1) -- (A);

\end{tikzpicture}


==> figures/subAppAlgo.tex <==

\begin{tikzpicture}  [-{Latex[length=1.5mm, width=1.5mm]}]
	\node[state] (A) {a};
	\node[state] (D) [below right =of A] {d};
	\node[state] (C) [above right =of D] {c};

	\path
			(A) edge [bend left] (C)
			(C) edge [bend left] (D)
			(D) edge [bend left] (A)
			(C) edge [bend left] (A);

\end{tikzpicture}

